Visualising Geographically-Embedded Origin-Destination Flows: in 2D and immersive environments

This thesis develops and evaluates effective techniques for visualisation of flows (e.g. of people, trade, knowledge) between places on geographic maps. This geographically-embedded flow data contains information about geographic locations, and flows from origin locations to destination locations. We explored the design space of OD flow visualisation in both 2D and immersive environments. We do so by creating novel OD flow visualisations in both environments, and then conducting controlled user studies to evaluate different designs.

==> content/2-related-work/interactions.tex <==

\section{Interactions}
\label{sec:related:interactions}



==> content/2-related-work/tasks.tex <==

\section{Task Identification}
\label{sec:related:tasks}



==> content/4-maptrix/0-introduction.tex <==
\section{Introduction}
\label{sec:maptrix:introduction}
There are two main approaches to visually presenting OD flows: \textit{flow maps} and \textit{matrices}. \textit{Flow maps} present origins and destinations on a map connected by lines or arrows. Whilst flow maps are intuitive and are well suited to show the flows from a single source, they quickly become cluttered and difficult to read when the number of commodity sources increases. For the \textit{matrix} approach, the most basic is the origin-destination (OD) matrix~\citep{Voorhees:2013cx} in which there is a row $r$ for each source (origin), a column $c$ for each destination, and a cell ($r$,$c$) shows the flow from source to destination. The drawback of the OD matrix is that geographical embedding of the sources and destinations is missing. This can be partly ameliorated by ordering the rows and columns by location, say east to west. More recently OD maps~\citep{Wood:2010be} have been suggested. These use a gridded two-level spatial treemap to cleverly preserve the approximate spatial (map) layout~\citep{Wood:2008gm}(see Section~\ref{sec:maptrix:od-map}).

==> content/colophon.tex <==
\pagestyle{empty}
\hfill
\vfill
\pdfbookmark[0]{Colophon}{Colophon}
\section*{Colophon}

This thesis was typeset with \LaTeXe.
It uses the \textit{Clean Thesis} style developed by Ricardo Langner.
The design of the \textit{Clean Thesis} style is inspired by user guide documents from Apple Inc.

Download the \textit{Clean Thesis} style at \url{http://cleanthesis.der-ric.de/}.

